Improving a Named Entity Recognizer Trained on Noisy Data with a Few Clean Instances

To achieve state-of-the-art performance, one still needs to train NER models on large-scale, high-quality annotated data, an asset that is both costly and time-intensive to accumulate. In contrast, real-world applications often resort to massive low-quality labeled data through non-expert annotators via crowdsourcing and external knowledge bases via distant supervision as a cost-effective alternative. However, these annotation methods result in noisy labels, which in turn lead to a notable decline in performance. Hence, we propose to denoise the noisy NER data with guidance from a small set of clean instances. Along with the main NER model we train a discriminator model and use its outputs to recalibrate the sample weights. The discriminator is capable of detecting both span and category errors with different discriminative prompts. Results on public crowdsourcing and distant supervision datasets show that the proposed method can consistently improve performance with a small guidance set.

==> tex/related_works.tex <==
\section{Related Works}
\noindent\textbf{Learning from noisy labels} is a actively researched topic in the Machine Learning community. \citet{goldberger2017training} proposed to model a class-level confusion matrix via the EM algorithm only using noisy labels, and use it to correct the loss function with noisy labels. \citet{hendrycks2018using} extend it adopting the confusion matrix with a small set of trusted data. The generalized cross entropy loss \citep{zhang2018generalized} is proposed to  balance between model convergence and noise-robustness, and is adopted in RoSTER \citep{meng2021distantly} to learn from distantly-supervised NER data. \citet{xu2019l_dmi} propose a information-theoretic loss function and prove its robustness to class-level label noise. \citet{shu2019meta} introduce a meta-learning framework to guidance the noisy learning by minimizing the meta-loss calculated with a small set of trusted data. \citet{han2018co} design a model-based sample selection strategy, where two differently-initialized models are used to select samples for each other. However, these methods are mostly designed for image classification, mainly about class level label noise. As we shown in Section \ref{sec:analysis}, the span error is severer in the noisy NER data. 



\noindent\textbf{Few-shot NER} is also related to our work. The goal is to train a NER model with limited labeled data. \citet{yang2020simple} propose to enhance the token representations in the testing set with tokens from a small set of labeled data. \citet{huang2020few} investigate the prototype-based method, noisy supervision pretraining and self-training techniques for few-shot NER. \citet{cui-etal-2021-template} formalize NER as a language model ranking problem and design prompts to identity named entities and their classes over all possible entity spans. \citet{lee2021good} shows that adding demonstration can improve the performance of few-shot NER. In our paper, we train the discriminator with a few clean instances, and use prompt tuning and demonstration from clean instances to improve the few-shot ability of the discriminator.


